Non-Uniqueness of Classical Inflationary Trajectories on a High-Dimensional Landscape

Motivated by the string landscape, inflation may happen on a high dimensional complicated potential. We propose a new way to construct some high dimensional random potentials, and study inflation on top of that, for up to 50-dimensions in field space. Especially, random bifurcations of classical inflationary trajectory are studied. It is shown that the bifurcation probability increases as a function of number of dimensions. Those random bifurcations are not consistent with observations, and dramatically limit the parameter space of inflation on a complicated landscape. For example, in 10 dimensions, only $10^{-3} \sim 10^{-6}$ of the parameter space volume leads to unique classical trajectories. The rest is ruled out by random bifurcations.

==> PaxHeader/msi_high_d.tex <==
30 mtime=1430053988.435402697
30 ctime=1430053988.435402697
30 atime=1430051216.741447494
161 LIBARCHIVE.xattr.user.com.dropbox.attributes=eJyrVkopyi9Iyq+IT8vMSc1Mic/JT07MUbJSqFbKTUzOyMwDiSWWlBSBhVISSxKBDKWwCl/DTPeyorDEQp98w/KwAB8/w4h0W1ul2tpaAMzuHKo

